High-Dimensional Learning in Finance

Recent advances in machine learning have shown promising results for financial prediction using large, over-parameterized models. This paper provides theoretical foundations and empirical validation for understanding when and how these methods achieve predictive success. I examine two key aspects of high-dimensional learning in finance. First, I prove that within-sample standardization in Random Fourier Features implementations fundamentally alters the underlying Gaussian kernel approximation, replacing shift-invariant kernels with training-set dependent alternatives. Second, I establish information-theoretic lower bounds that identify when reliable learning is impossible no matter how sophisticated the estimator. A detailed quantitative calibration of the polynomial lower bound shows that with typical parameter choices, e.g., 12,000 features, 12 monthly observations, and R-square 2-3%, the required sample size to escape the bound exceeds 25-30 years of data--well beyond any rolling-window actually used. Thus, observed out-of-sample success must originate from lower-complexity artefacts rather than from the intended high-dimensional mechanism.

==> preamble.tex <==
\RequirePackage[english]{babel}
%\RequirePackage{authblk}
\RequirePackage{amsthm}
\RequirePackage{amsmath}
\RequirePackage{graphicx}
\RequirePackage[countmax]{subfloat}
\RequirePackage{subfig}
\RequirePackage{natbib}
\RequirePackage{setspace}
%\RequirePackage[left=1.25in, right=1.25in, top=1.2in, bottom=1in]{geometry} % use with 11pt
\RequirePackage{geometry} % use with 11pt
\RequirePackage{tabularx}
\RequirePackage{booktabs}
%\usepackage{bm}
\RequirePackage{mathtools}
\mathtoolsset{mathic=true,showonlyrefs} 
\RequirePackage{tikz}
\usepackage{pgfplots}

% \RequirePackage{enumitem}
%------------ from Hasan --------------
\usepackage{setspace}
\usepackage{multirow}
\usepackage{adjustbox}
\usepackage{lscape}
\usepackage{booktabs}
\usepackage{threeparttable}
\usepackage{adjustbox}
\usepackage{pdflscape}
\usepackage{array}
\usepackage{siunitx}
\sisetup{
  round-mode = places,
  round-precision = 3,
  table-format = 2.3,
  group-four-digits = false
}

\usepackage[toc]{appendix} % Handles appendices and their TOC inclusion

%---------------------------------------------
\RequirePackage[sf,bf]{titlesec}
\RequirePackage{fancyhdr}
\RequirePackage{caption}
\captionsetup{labelfont = bf,format = hang, justification = justified, font = footnotesize}

\RequirePackage[original]{abstract}

\RequirePackage{microtype}

\bibliographystyle{agsm}

\renewcommand*{\bibfont}{\small}
\setlength{\bibsep}{0pt}

% \newtheorem{definition}{Definition}
% \newtheorem{theorem}{Theorem}
% \newtheorem{assumption}{Assumption}
% % \newtheorem{lemma}{Lemma}
% \newtheorem{proposition}{Proposition}
% \newtheorem{corollary}{Corollary}
% \newtheorem{remark}{Remark}

\allowdisplaybreaks[4]

% \newcommand{\eqldist}{\overset{\scriptscriptstyle d}{=}}
% \newcommand{\eqlas}{\overset{\scriptscriptstyle \mathit{a.s.}}{=}}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\N}{\mathbb{N}}
% \newcommand{\E}{\mathbb{E}}
% \DeclareMathOperator{\cov}{cov}
% \DeclareMathOperator{\diag}{diag}
% \DeclareMathOperator{\tr}{tr}
% \DeclareMathOperator*{\plim}{plim}
% \newcommand\norm[1]{\left\lVert#1\right\rVert}
% \newcommand\dotprod[1]{\langle#1\rangle}

\numberwithin{equation}{section}
% \newtheorem{lemma}{Lemma}[section]


\geometry{left=1in, right=1in, top=1in, bottom=1in}
\RequirePackage{amssymb}
\RequirePackage{mlmodern}
\RequirePackage[scr=boondoxo, bb=pazo, frak=boondox]{mathalpha}
\RequirePackage{bm}
%\newcommand{\transp}{\intercal}

\makeatletter
\newcommand*{\transp}{
	{\mathpalette\@transp{}}
}
\newcommand*{\@transp}[2]{
	\raisebox{\depth}{$\m@th#1\intercal$}
}
\makeatother

\thinmuskip=2.5mu
\medmuskip=3mu plus 1mu minus 3mu
\thickmuskip=3.5mu plus 2.5mu
\setstretch{1.05}


\RequirePackage{hyperref}
\hypersetup{%
	colorlinks = true,
    linkcolor = blue,
     anchorcolor = blue,
     citecolor = blue,
     filecolor = blue,
     urlcolor = blue,
}

% \usepackage{xcolor}
% \usepackage[colorlinks=true, urlcolor=blue, linkcolor=blue]{hyperref}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usepackage{ifluatex}

% \newtheorem{assumptionalt}{Assumption}[assumption]

% Custom commands
% \newcommand{\norm}[1]{\left\|#1\right\|}
% \newcommand{\abs}[1]{\left|#1\right|}
% \newcommand{\R}{\mathbb{R}}
% \newcommand{\E}{\mathbb{E}}
\newcommand{\F}{\mathcal{F}}
\newcommand{\tF}{\tilde{\F}}
\newcommand{\X}{\mathcal{X}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\ep}{\epsilon}
\newcommand{\prob}{\mathbb{P}}
\newcommand{\Hn}{H_n}
\newcommand{\Ld}{L_d}
\newcommand{\fn}{\hat{f}_n}
\newcommand{\fstar}{f_*}
\newcommand{\Rn}{R_n}

\DeclareMathOperator*{\argmin}{arg\,min}

\usepackage{stackengine}
\newcommand\toas{\altxrightarrow{a.s.}}
\newcommand\todist{\altxrightarrow[-1pt]{d}}
\newcommand\toprob{\altxrightarrow[-1pt]{p}}
\newcommand\altxrightarrow[2][0pt]{\mathrel{\ensurestackMath{\stackengine%
			{\dimexpr#1-7.5pt}{\xrightarrow{\phantom{#2}}}{\scriptstyle\!#2\,}%
			{O}{c}{F}{F}{S}}}}

\usepackage{tikz}
\usetikzlibrary{matrix, backgrounds}
